VeriSplit: Secure and Practical Offloading of Machine Learning Inferences across IoT Devices

Many Internet-of-Things (IoT) devices rely on cloud computation resources to perform machine learning inferences. This is expensive and may raise privacy concerns for users. Consumers of these devices often have hardware such as gaming consoles and PCs with graphics accelerators that are capable of performing these computations, which may be left idle for significant periods of time. While this presents a compelling potential alternative to cloud offloading, concerns about the integrity of inferences, the confidentiality of model parameters, and the privacy of users' data mean that device vendors may be hesitant to offload their inferences to a platform managed by another manufacturer. We propose VeriSplit, a framework for offloading machine learning inferences to locally-available devices that address these concerns. We introduce masking techniques to protect data privacy and model confidentiality, and a commitment-based verification protocol to address integrity. Unlike much prior work aimed at addressing these issues, our approach does not rely on computation over finite field elements, which may interfere with floating-point computation supports on hardware accelerators and require modification to existing models. We implemented a prototype of VeriSplit and our evaluation results show that, compared to performing computation locally, our secure and private offloading solution can reduce inference latency by 28%--83%.

==> plots/cdf_layerworks.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/lazy_workers_cdf-2.pdf}
    \caption{Cumulative Distribution Functions (CDFs) of different verifiers in detecting a lazy worker that (1) uses a MobileNet (left) and (2) quantizes a VGG16 model to 16-bit floating-point precision (right). Each point $(n, p)$ on a CDF curve indicates a probability $p$ of detecting the lazy worker with inferences less than $n$. We use ``(x\%)'' to mark that a verifier randomly check an inference with a probability of x\%. }
    \label{fig:cdf_laze_workers}
\end{figure*}



==> plots/com_overhead.tex <==
\begin{figure}
    \centering
\includegraphics[width=\columnwidth]{figures/Com_Overhead.pdf}
    \caption{Communication overhead of VeriSplit for verifying inference on a GPU, Jetson Nano and an Apple M1 pro laptop when offloading the image classification task using VGG16. \ZW{explain the specifications.}}
    \label{fig:verisplit_communication_overhead}
\end{figure}


==> plots/latency-breakdown-v2.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/latencyBreakdownV2.pdf}
    \caption{Latency breakdown of selected GPU offloading experiments. Operations in hatch patterns happen on the worker, while plain bars are operations on the verifier side. Compared to the baseline, offloading multiple inferences concurrently (multi-threading) incurs resource contention on the worker. To conduct inference with a smaller threshold, the worker has to pad the inference to use bigger batch sizes. Therefore, the worker takes longer in processing inferences and generating proofs.}
    \label{fig:latency-breakdown}
\end{figure*}

==> plots/latency_breakdown.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/latency_breakdown.pdf}
    \caption{Latency Breakdown \ZW{Switch labels of these two rows}}
    \label{fig:my_label}
\end{figure*}

==> sections/partial-verification-details.tex <==

\section{Partial Verification for Integrity}
\label{sec:partial-verification}

In this section, we explained how to verify the results of a single layer. However, the simple Merkle tree only supports checking each layer's results in their entirety. The inputs and outputs of one network layer can still be quite large, and verifying them requires significant computation.  Instead, \emph{partial} verification  intuitively can be beneficial to reduce the overhead since the verifier would need to check a subset of values. 

Directly reducing a simple Merkle for partial verification is inefficient. The worker needs to generate proof with entire layer inputs and outputs (as the basis of the Merkle tree leaf nodes), even if the verifier only checks a small subset. If the verifier wants to verify a tiny portion of \emph{every} layer, the worker needs to send \emph{all} values! To solve this issue, we extend the original Merkle tree with fine-grained leaf nodes of smaller content sizes, reducing proof sizes and communication overhead. \Cref{fig:slicing-units} visualizes an example of \verisplit{}'s slicing algorithm, which we will explain next.


\begin{figure}[t]
    \centering
    \input{plots/layer-slicing.tex}
    \caption{An example comparison between \verisplit{}'s disjoint slicing mechanism and the continuous approach. We select the unit size to be 2x2. We color-code disjoint units and mark continuous units by their content. For continuous slicing, we only show slicing a 3x3 matrix due to limited spaces. The red box indicates one possible region verifiers may choose to check. After slicing, the Merkle tree adds extra leaf nodes, as shown in the transition from one hash $h_m$ of the original matrix into 4 more leaves ($h_1$--$h_4$). }
    \label{fig:slicing-units}
\end{figure}


\subsection{Slicing Verify Units}
It turns out that slicing layers' outputs into smaller units involves many trade-offs and deliberations. At one extreme, we can single out every element in the matrix into one unit. 
This provides fine granularity for partial verification since verifiers can choose arbitrary regions. However, it is impractical because of the large dimensions of layer results (e.g., certain VGG16 layers have outputs of 224x224x64). The more units we have, the larger the Merkle tree will be, and the worker needs to compute significantly more hashes to create the commit during inference time. 
Instead, we choose a fixed unit size, balancing the complexity of the Merkle tree and the flexibility of partial verification (\Cref{sec:configure-verify-ratio} explains how to choose this value). 

In \verisplit{}, we employ a disjoint slicing method to separate large matrices into smaller verify units. \Cref{fig:slicing-units} visualizes this slicing method compared with continuous alternatives. Disjoint slicing generates less number of units (we can not enumerate continuous units in a 4x4 matrix due to limited spaces), leading to less computation in the Merkle tree construction during inference. The compromise with disjoint slicing is that, during verification, the worker might need to include more neighboring units in the proof. For example, if the verifier selects the region in the red box, the worker needs to include all 4 slices since the exact region is not included in any individual Merkle tree leaf node. 


Certain layer types cannot benefit from unit slicing to reduce the computation overhead. For example, dense layers with softmax activation are often used in the final prediction layer. To verify softmax, the verifier needs to gather all layer inputs and outputs, eliminating the benefit of partial verification. \verisplit{} thus reverts to full layer verification for those layers. Fortunately, many computationally demanding layers can benefit from partial verification (such as convolution layers, who take up over 90\% of all computations in certain CNN models~\cite{chen2016eyeriss, li2017convolution-pruning, lin2017predictivenet}).

\subsection{Tunable Verification}
\label{sec:configure-verify-ratio}

\verisplit{} utilizes a configurable knob (verify ratio) to decide the size of individual verify units. If the verifier wants to enable partial verification as fine-grain as 1\% (by setting this as the verify ratio), the worker slices each layer's results into at least 100 units. We can then calculate the unit size accordingly. The verifier can select a new value for every offloading request. This helps the verifier to adjust partial verification ratios based on the predicted arrival rates of new inferences. For scenarios where new inferences are rare, the verifier can set a higher ratio for individual offloads or maybe even perform full verification. On the other hand, if there are a large number of inferences consistently arriving, the verifier can set a smaller verify ratio to preserve resources while retaining a high probability of catching malicious workers.




==> tables/highlevel_comparison.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{cccccc}
    \toprule
    \toprule
         Verification & Communication  & Computation 
&Storage Overhead  &  Detection Latency & False Negative  \\
        Method  & Overhead &  Overhead 
&in Asynchronous Setup & on Lazy Workers & Error (FNE)\\
        \midrule
         Slalom~\cite{tramer2018slalom} & High & High & High&High& Very Low\\
         Top-Layer Verifier & Low & High & Task-Dependent&High&High\\
         Class Verifier & Low & High & Low&High& High \\
         \textbf{VeriSplit (ours)} & \textbf{Low} & \textbf{Low} & \textbf{Low}& \textbf{Low}& \textbf{Tunable}\\
          \toprule
    \end{tabular}
    \caption{Qualitative comparisons between verification methods for checking inference integrity (Definition~\ref{def:integrity}) when offloading ML inferences to IoT workers. Except that a class verifier is only suitable when offloading classification tasks, others are designed for general ML tasks. False Negative Error refers to that a verifier claims integrity but is actually violated. FNE is tunable in VeriSplit because it performs partial verification for the model's internal activations (\Cref{sec:partial-verification}).}
    \label{tab:qualitative-comparisons-of-baselines-and-verisplit}
\end{table*}

==> tables/optimization-impact.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{M{22mm}|M{17mm}|M{13mm}|M{14mm}}
    \toprule 
    \toprule 
    {Runtime Options} & {Network Comm. (MB)} & {Latency (ms)} & {Verifier CPU Load}
    \\
    \hline
    \hline
    Baseline & $2.66 \pm 0.26$ & $1993 \pm 148$ & 0.63 \\
    % \hline
    No Caching & $2.66 \pm 0.26$ & $3158 \pm 174$ & 0.77 \\
    % \hline
    No Compression & $3.75 \pm 0.38$ & $2012 \pm 224$ & 0.57\\
    % \hline
    Verify 10\% & $ 13.44 \pm 2.35$ & $2933 \pm 537$ & 1.04 \\
    % \hline
    Lower Threshold & $2.67 \pm 0.25$ & $2822 \pm 148$ & 0.45 \\
    \bottomrule
    \end{tabular}
    \caption{Performance impact of various \verisplit{} runtime configurations. In the baseline, we enable all optimizations, verify 1\% of the network, and use \Ltwo{} with batch size 1 as the threshold. The lower threshold alternative uses batch size 16 (c.f. \Cref{tab:threshold-attacks}), which requires padded inference due to batch size mismatches.}
    \label{tab:optimization-impact}
\end{table}

==> tables/platform-comparison.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{M{17mm}|M{9mm}|M{9mm}|M{14mm}|M{14mm}}
    \toprule 
    \toprule 
    \multirow{3}{13mm}{Worker Platform} & \multicolumn{2}{c|}{Verifier} & \multirow{3}{8mm}{Latency (ms)} & \multirow{3}{14mm}{Throughput (infer./sec)} 
    \\
    \cline{2-3}
    &  Threads & CPU Load & & \\
    \hline
    \hline 
    \multirow{2}{10mm}{Local (RPi 4)} & 1x & 1.01 & $5756 \pm 1079$ & 0.17  \\
    \cline{2-5}
     & {4x} & {\textbf{2.61}} & {$\bm{1746 \pm 13}$} & {\textbf{0.57}}\\ 
    \hline
    \multirow{2}{8mm}{GPU} & {1x} & {\textbf{0.63}} & {$\bm{1993 \pm 148}$} & {0.51}  \\
    \cline{2-5}
    & 4x & 1.25 & $3797 \pm 673$ & {\textbf{1.07}}  \\ 
    \hline
    \multirow{2}{10mm}{Apple M1 Pro}& 1x & 0.57 & $1891 \pm 295$ & 0.53  \\
    \cline{2-5}
    & 4x & 1.23 & $3671 \pm 891$ & 1.06  \\ 
    \hline
    Jetson Nano & 1x & 0.11  & $9024 \pm 409$ & 0.11 \\
    \bottomrule
    \end{tabular}
    \caption{Performance comparison between local inferences and \verisplit{} offloading to various hardware platforms. The average end-to-end latency includes both inference and verification times. Even single-thread GPU offloading offers comparable latency with multi-threaded local inference on the verifier. Offloading multiple inferences in parallel (multi-threading) further improves inference throughput while keeping CPU load at half of local inference utilization.}
    \label{tab:platform-comparison}
\end{table}

==> tables/throughput-backup.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{lcc}
    \toprule 
    \toprule
    \multicolumn{1}{c}{Worker Platform} & Throughput & CPU Load\\
    \multicolumn{1}{c}{} & (Inferences/sec) & ($\times$ 100\%)\\
    \midrule
      GPU &  0.51 & 0.63\\
      GPU (w/ padding)   &  0.36 & 0.45\\
      GPU (10\% verification)   &  0.34 & 1.04\\  
      GPU (no caching)   &  0.32 & 0.77\\  
      GPU (multi-threads)   &  1.07 & 1.68\\ 
      GPU (no data compression)   &  0.50 & 0.57\\ 
      Jetson Nano   &  0.11 & 0.11\\ 
      Apple M1 pro  &  0.54 & 0.68\\ 
      \midrule
      Local (no cap) & 0.17 & 1.01\\
      Local (1x thread) & 0.58 & 2.61\\
      \bottomrule\\
    \end{tabular}
    \caption{Comparing the throughput (inferences / sec) of offloading devices when asked to predict the lables of 256 images ($224\times224\times3$) with a VGG16 model. \ZW{TODO: explain the specification of each row.}}
    \label{tab:inference-throughput-backup}
\end{table}

==> tables/throughput.tex <==
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{M{15mm}||M{3mm}M{20mm}M{14mm}M{13mm}M{14mm}M{18mm}|M{6mm}M{10mm}|M{3mm}M{14mm}}
    \toprule 
    \multirow{2}{10mm}{Worker Platform} & \multicolumn{6}{c|}{GPU} & \multirow{2}{6mm}{Jetson Nano} & \multirow{2}{10mm}{Apple M1 Pro} & \multicolumn{2}{c}{Local} \\
    \cline{2-7} \cline{10-11}
    & - & Low Threshold & Verify 10\% & No Cache & 4x Threads & No Compress. & & & - & 1x Thread \\
    \midrule 
    Throughput (infer./sec) & 0.51 & 0.36 & 0.34 & 0.32 & 1.07 & 0.50 & 0.11 & 0.54 & 0.58 & 0.17 \\
    \midrule 
    Verifier CPU Load & 0.63 & 0.45 & 1.04 & 0.77 & 1.68 & 0.57 & 0.11 & 0.68 & 2.61 & 1.01 \\
    \bottomrule
    % \multicolumn{1}{c}{Worker Platform} & Throughput & CPU Load\\
    % \multicolumn{1}{c}{} & (Inferences/sec) & ($\times$ 100\%)\\
    % \midrule
    %   GPU &  0.51 & 0.63\\
    %   GPU (w/ padding)   &  0.36 & 0.45\\
    %   GPU (10\% verification)   &  0.34 & 1.04\\  
    %   GPU (no caching)   &  0.32 & 0.77\\  
    %   GPU (multi-threads)   &  1.07 & 1.68\\ 
    %   GPU (no data compression)   &  0.50 & 0.57\\ 
    %   Jetson Nano   &  0.11 & 0.11\\ 
    %   Apple M1 pro  &  0.54 & 0.68\\ 
    %   \midrule
    %   Local (no cap) & 0.17 & 1.01\\
    %   Local (1x thread) & 0.58 & 2.61\\
    %   \bottomrule\\
    \end{tabular}
    \caption{Comparing the throughput (inferences / sec) of offloading devices when asked to predict the lables of 256 images ($224\times224\times3$) with a VGG16 model.}
    \label{tab:inference-throughput}
\end{table*}
